Polyadic Quantum Classifier

We introduce here a supervised quantum machine learning algorithm for multi-class classification on NISQ architectures. A parametric quantum circuit is trained to output a specific bit string corresponding to the class of the input datapoint. We train and test it on an IBMq 5-qubit quantum computer and the algorithm shows good accuracy --compared to a classical machine learning model-- for ternary classification of the Iris dataset and an extension of the XOR problem. Furthermore, we evaluate with simulations how the algorithm fares for a binary and a quaternary classification on resp. a known binary dataset and a synthetic dataset.

==> texfiles/cabbrev.tex <==
\section{Circuit abbreviations}
\label{cabbrev}
To make our circuits more compact and readable we use the following abbreviations:


\newcolumntype{C}{ >{\centering\arraybackslash} m{3cm} }

\begin{center}


	\begin{tabular}{ c c c }
			\qc{&\qw&\sx&\qw&\qw&\qw}  & $\equiv$ & \hspace{-10mm}\qc{&\qw&\SQRTX& \qw&\qw} \\ \\
	\qc{\losange&\qw&\qw&\qw&\qw}  & $\equiv$ & \hspace{-10mm}\qc{&\ket{0}\hspace{4mm}&\qw&\sx& \qw&\qw} \\ \\
	\parbox[c]{2.5em}{\qc{&\qw& \qw& \qw&\qw&\qw\filledtriangleright\qwx[2]&\qw &\qw&\qw&\qw \\ &&\\
			&  \qw& \qw&  \qw& \qw&\qw\filledtriangleright &\qw&\qw&\qw&\qw&& }} & $\equiv$ &
	\parbox[c]{8em}{\qc{&\qw&\qw&\qw&\ctrl{1}&\qw &\sx& \qw& \qw& \qw& \qw \\
			&\qw&\qw&\qw&\ctrl{0}&\qw & \sx& \qw& \qw& \qw& \qw} }    \\ \\
%	\qc{&\qw&\gate{\theta}&\qw&\qw} & $\equiv$ & \qc{&\qw&\gate{R_z(\theta)}&\sx&\qw} \\ \\
		\qc{&\qw&\gate{\phi}&\qw&\qw} & $\equiv$ & \hspace{-8mm}\qc{&\qw&\gate{Z_\phi}&\sx&\qw&\qw}
%	\qc{&\qw&\qw& \gate{\theta_0|\theta_1}& \qw& \qw} & $\equiv$ & \hspace{-1.2cm}\qc{&\qw&\qw& \gate{\theta_0 } &\gate{ \theta_1}& \qw& \qw}
\end{tabular}
\end{center}


==> texfiles/conclusion.tex <==
\section{Conclusion}
This is reminiscent of how machine learning evolved towards deep learning with the advent of new computational capabilities

We tested many different circuit architectures, and tried various learning tricks; too many to be fully incorporated in this paper.
Therefore, we discuss only the most interesting examples for each dataset, trying to highlight their peculiarities and cast light on some technique that we found successful.


\textit{---need more in the paper before writing this}
\textit{we haven't demonstrate quantum advantage: our algorithm fares well but haven't surpass its classical counterparts.}
\tdok{This sentence must go. From the very beginning of the manuscript one has to very clearly say that the scope here is a proof of concept of a polyadic classification using quantum processors. There is no intention to demonstrate quantum advantage and there are no claims about how interference plays a role. This is a toy model, and it is important to state it}
\jk{Yep sorry this a random draft, I should have included it, conclusion has to written when the paper is almost ready}
Now comes a greater challenge: generalize and demonstrate the learning algorithm for problems of higher magnitude ---using as many qubits as needed--- and show that it can perform some tasks of importance with a lower algorithmic complexity.


==> texfiles/conversation.tex <==

\section*{Anotations example}

\td{Annotations by Tommaso}

\me{Annotations by Ewan}

\kj{Annotations by Joaqu\'{i}n}


  \section*{\td{Major points and notes to keep in mind}}
\td{I believe the message has to be shaped around certain key points:
	\begin{itemize}
		\item How does this work differ from previous works in supervised classification with quantum processors?
		\kj{Answering in full this question would need to do a complete state of the art of the domain. An alternative option is to do attribution with citations: each time you introduce something you say where you get the idea from. This avoid to have to say: these and these papers did the thing differently}
		\item What are the claims
		\kj{I assume that this means "what is original in this work". I think the abstract summarize this point pretty well. Even short summary: an algorithm, 3 experiments.
		}\\ \\
		\kj{Discussion, main strengths of the algorithm compared to previous qml algorithms for supervised learning:
		\begin{enumerate}
			\item polyadic classification (vs binary)
			\item it is noise resilient
			\item it fares well compared to classical ML
			\item it need less resources (ie qubits, gates, shots)
			\item previous point could mean lower algorithmic complexity
		\end{enumerate}
	Point 1 can be claimed to some extent (you can always do an n-ary classification with many binary ones. So this goes to point 4). \\
	Points 2, 3, 4  cannot be claimed in general, it can only be: in these experiments the algorithm was noise resilient, fared well compared to CML, and needed few resources. That's why ML community uses the same test datasets (Iris, MNIST, CIFAR, ImageNet, etc...), to be able to compare their results. And that's why we worked on the iris dataset. \\
	Point 5 is difficult to claim. Usually ML community do not talk much about that. They say my algorithm worked well on this problem, it needed that many hours of compute time.\\
	However, we need to be able to say something someday on this point. This is how a QML algorithm could prove Q advantage. That's why I am studying complexity theory of ML. Maybe there is no answer for this. Maybe it would only happen by an empirical proof: for this problem, this QML algorithm on this quantum computer fares better than any existing CML algorithm on the most powerful C computer. This means that if we run more and more complex problems using the full potential of the QPUs of the day, we might someday reach QML advantage (over CML). This is more a rationale for series A than something for a scientific paper.
}
	\item What are NOT the claims
	\kj{This is an infinite space. We can say what we think is missing and will our future work\\
		To do:
	\begin{itemize}
		\item try to solve problems with higher feature dimensions (using more qubits and more gates)
		\item design optimizers  better at minimizing quantum loss functions
	\end{itemize}
Explicit no claims:
	\begin{itemize}
		\item we do not claim quantum advantage
		\item we do not claim the algorithm work for something else than these datasets
	\end{itemize}}
	\item Work on the paper structure, now it is weak. Once the claims are laid out, we can build a consistent structure. \\
	\kj{Ongoing work: the claims are an algorithm + 3 experiments, so this is structure of the paper}
	\item State from the beginning that the goal is to run this on a quantum computer\\
	\kj{Agree, however this is not a the goal, the goal is to have a algorithm that could run on a NISQ device. It happened that for the iris it could run on an ibmq, , so we decided to do it}
	\item Have a detailed section where all details are explained in a rigorous fashion
	\item Detailed description of the quantum circuit
	\item Detailed description of the processors used, error rates, time it took to run the algorithm and related information\\
	\kj{the 3 points above belong to the experiments part}
	\item Can we find a comparison with classical methods? What is the best way to run a fair comparison, against what methods, and what metrics of goodness do we need and use?\\
\kj{The standar metric (ML community) to compare the quality of classifier algorithms is accuracy. \\ ML community organize annual events where they compare their }
	\item Who are we talking to? The physics community? The machine learning community? The investors (i.e., does not matter who we talk to in scientific communities)? This choice motivates the structure and language of the manuscript. As it is now, it is not well fit for the general physics community.\\
	\kj{we talk to the quantum computing algorithms community and more specifically to the quantum machine learning community. This is a multidisciplinary community that includes people from physics, TCS and Machine Learning. We need to avoid a language targeted to only one discipline. }
\end{itemize}}




==> texfiles/discussion.tex <==
\section{Discussion}

\textbf{What is good ?}
\begin{enumerate}
    \item $\checkmark$ We find solutions for data of different shapes, with non-linear decision boundaries.
    \item $\checkmark$ Resilience to noise and low number of shots.
    \item Low overfitting.
\end{enumerate}

\textbf{What is missing/bad ?}
\begin{enumerate}
    \item Need to improve/specialize the optimizer.
    \begin{itemize}
        \item $\checkmark$ We lack a statistical approach on the choice of shots.
        \item $\checkmark$ Less shots = randomize algorithm + less complexity.
        \item $\checkmark$ We need to improve the gradient approximation estimation cite papers.
    \end{itemize}
    \item We need to increase the dimensionality and the number of qubits.
    \item We lack a theoretical study to support our design choices.
    \item We should understand better the parameter space.
    \item We are close, but always below, classical models.
\end{enumerate}

\textbf{What would be interesting to add ?}
\begin{enumerate}
    \item Run on QPU a bigger dataset (using minibatches).
    \item Try other encoding functions (for both features and model parameters), for instance
     sigmoids.
     \item $f(t) = \theta$ this includes parameter sharing
\end{enumerate}

We step out now from the experimental process, to discuss the results we gathered.
First of all, we point out that, for each experiment with quantum classifiers, the quantum program was able to learn non-linear shapes and that we obtained good test scores, compared to a classical model.
This suggests that, at least in principle, this family of machine learning models is flexible enough to be applied for polyadic classification.

Furthermore, thanks to the experiment with the Iris flower dataset, discussed in section \ref{ssec:iris-exp}, we prove by evidence that learning with a small dataset is possible even on NISQ architectures and that we can obtain accurate predictions even with as little as 300 shots per samples.
On top of the latter, the trained model is resilient to a change of hardware, as the accuracy confidence intrerval from Fig. \ref{fig:iris-ibmq-circuit} is narrow.

From the experimental results, it appears that quantum classifiers are not prone to overfit. In machine learning, emph{overfitting} is defined as having a very low loss value on the training set, but a poor performance on independent test data.
It is not the case here, as the training accuracy is always very close to what we observe on the test set.

Nonetheless, we encountered some problems, which should be addressed in future research.
First of all, the optimization procedure should be improved.
In fact, we lack a statistical approach on the choice of shots during training and we should find a way to use gradient based methods even on hardware.
The first one could be helpful to reduce the randomness while approaching a possible solution, or to increase it to get away from, local minima.

The gradient, on the other hand, would be necessary to upscale our circuits, as gradient-free methods are known to drastically loose performance if the parameter space has high dimensionality.
It could be helpful to explore methods to approximate the gradient as proposed in \cite{crooks2019gradients,schuld2018gradients}.

Then, we should investigate wheter this algorithm works with higher dimensional data and, similarly, with an higher number of qubits.
Data dimensionality is important as most interesting applications of machine learning rely on huge feature spaces.
In parallel, an higher number of qubits would be necessary to get an advantage over classical computers and motivate the use of QPUs in machine learning.

% The next milestone in quantum machine learning would thus be the design of a specific optimization algorithm, able to account for intrinsic randomness and to adjust the number of shots and the search direction accordingly.

%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=\linewidth]{figures/qml-iris-predictions.pdf}
%
%	\caption{Decision boundaries for Iris dataset of the quantum circuit in Figure \protect\ref{fig:iris-ibmq-circuit}.
%	The axes are the first two principal components of the training dataset, over which all samples are projected.
%	Figure shows the predicted label of each point in the plane color-coded in the background.
%	In the forecground, we represent both test samples and training samples, the former highlighted by ther greater size.
%	The model learns nontrivial decision boundaries and do not seems to overfit.}
%	\label{fig:iris-decision}
%\end{figure}

